One vertex spin-foams with the Dipole Cosmology boundary

We find all the spin-foams contributing in the first order of the vertex expansion to the transition amplitude of the Bianchi-Rovelli-Vidotto Dipole Cosmology model. Our algorithm is general and provides spin-foams of arbitrarily given, fixed: boundary and, respectively, a number of internal vertices. We use the recently introduced Operator Spin-Network Diagrams framework.

==> One vertex spin-foams with the Dipole Cosmology boundary/00_preambula.tex <==
% Czcionka
\usepackage[utf8]{inputenc}
\usepackage[OT4]{fontenc}

% Pakiety Podstawowe
%\usepackage{amsmath,amsthm,latexsym,amssymb,amsfonts}
\usepackage{iopams}
%\usepackage{showlabels}
%\usepackage{eufrak}
%\usepackage{polski}
\usepackage{enumerate}
\usepackage{graphicx}
\usepackage{calc}
\usepackage{colordvi}
\usepackage{color}
\usepackage{vmargin}
\usepackage{array}
% Można by dodać poniższy, gdyby istniał
%\usepackage{LQC-symbols}
\usepackage{subfig}

% DEBUG
%\usepackage[normalem]{ulem}

%****************************************************%
%*****************    Komendy    **********************%
%****************************************************%


%**************   1. Tryb matematyczny:   ***************%


% Brakety:
\newcommand{\bra}[1]{\left\langle#1\right|}
\newcommand{\ket}[1]{\left|#1\right\rangle}
\newcommand{\braket}[1]{\left\langle{#1}\right\rangle}
\newcommand{\melement}[3]{\braket{#1\left|#2\right|#3}}


% Indeksy dolne pisane tekstem zwykłym
\newcommand{\gr}{{\rm gr}}
\newcommand{\scl}{{\rm sc}}
\newcommand{\tot}{{\rm tot}}
\newcommand{\phys}{{\rm phys}}
\newcommand{\kin}{{\rm kin}}
\newcommand{\KKL}{\mathrm{KKL}}
\newcommand{\AL}{\mathrm{AL}}
\newcommand{\DC}{\mathrm{DC}}
\newcommand{\LQG}{\mathrm{LQG}}
\newcommand{\diff}{\mathrm{diff}}
\newcommand{\inn}{\mathrm{in}}
\newcommand{\out}{\mathrm{out}}


% Symbole funkcji lub operacji:
\renewcommand{\tr}{\mathrm{Tr}}
\newcommand{\inv}{\mathrm{Inv}}

%%Symbole matematyczne
\newcommand{\id}{\idd}	%wybór wersji Id
%%Trzy wersje Id :
	\newcommand{\idd}{\mathbf{1}}
	\newcommand{\iddd}{\mathbb{1}}
	\newcommand{\idddd}{\mathbb{I}}
%% dalsze:
\newcommand{\im}{\dot\imath}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\pd}{\partial}


% Zmiany stylu pisma:
\newcommand{\K}[1]{\mathbb{#1}}	% Ciała matematyczne
\newcommand{\T}[1]{\mathcal{#1}}	% Zbiory otwarte, transformaty i funktory...

\newcommand{\N}{\T{N}}	% Funkcja cylindryczna (czy też: spinnetwork)


% Oznaczenia przestrzeni Hilberta
\newcommand{\Hil}{\mathcal{H}}
\newcommand{\Hal}{\Hil_{\mathrm{AL}}}
\newcommand{\Hd}{\Hil_{\mathrm{DC}}}
\newcommand{\Hgr}{{\Hil_{\gr}}}
\newcommand{\Hsc}{{\Hil_{\scl}}}
\newcommand{\Htot}{{\Hil_{\tot}}}
%
\newcommand{\Hgrb}{{\Hil_{\gr,B}}}
\newcommand{\Hphys}{{\Hil_{\phys}}}

% Konstrukcja przestrzeni Hilberta: operacja Span (dwie wersje ;)
\newcommand{\Span}{{\rm Span}}
%\newcommand{\spann}[2]{\begin{array}{c}\mathrm{span}\\#1\end{array}\left(#2\right)}
\newcommand{\spann}[2]{\begin{array}{c}span\\ \;_{\substack{#1}}\end{array} \left(#2\right)}


% Więzy
\newcommand{\Cgr}{{\widehat{C_{\gr}}}}
\newcommand{\Csc}{{\hat{C}_{\scl}}}
\newcommand{\Ctot}{{\hat{C}_{\tot}}}



%Odstępy w trybie matematycznym
\newcommand{\tab}{\qquad\qquad}
\newcommand{\taab}{\tab\tab}



%inne, których nie używam raczej...
\newcommand{\omicron}{{\cal I}}
%
\newcommand{\ppi}{{\scriptstyle\Pi}}
\newcommand{\F}{{\mathcal F}}



%*************   2. Tryb niematematyczny:   **************%

% Środowiska
\newtheorem{lm}{Lemma}
\newtheorem{thm}[lm]{Theorem}
\newtheorem{df}{Definition}
	%testowe
%	\newtheorem{comment}{Comment}


%Notka na marginesie:
\newcommand{\mnote}[1]{{\Red{*}}\marginpar{%
      \vskip-\baselineskip
      \raggedright\footnotesize
      \itshape\hrule\smallskip\tiny{\Red{#1}}\par\smallskip\hrule}}



% odsyłacze:
\newcommand{\reef}[1]{(\ref{eq:#1})} %do równania
\renewcommand{\fref}[1]{figure~\ref{fig:#1}} %do obrazka
\renewcommand{\sref}[1]{section~\ref{sc:#1}} %do rozdziału
\renewcommand{\Fref}[1]{Figure~\ref{fig:#1}} %do obrazka
\renewcommand{\Sref}[1]{Section~\ref{sc:#1}} %do rozdziału



% Jeszcze kilka wygonych definicji matematycznych

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\ba{\begin{eqnarray}}
\def\ea{\end{eqnarray}}
\def\lp{{\ell}_{\rm Pl}}
\def\g{\gamma}

\newcommand{\s}[1]{{#1}^{(s)}}






==> One vertex spin-foams with the Dipole Cosmology boundary/4_podsumowanie.tex <==

%Podsumowanie
\section{Summary, conclusions and outlook}
We presented a general algorithm for finding all spin-foams with given boundary graph in given order of vertex expansion. We applied this algorithm to the spin-foam cosmology model \cite{SF_cosmology} and found all contributions in first order of vertex expansion which are compatible with generalization of EPRL vertex \cite{SFLQG}. We expect that for a generic state the vertex used in \cite{SF_cosmology} gives the main contribution to the transition amplitude. This scenario needs however more thorough calculations and we leave it for further research.

The calculation we presented illustrates an application of OSN diagrams. The strength of this formalism lies in simplifying the classification of 2-complexes -- listing those with given properties (such as order of vertex expansion or structure of boundary graph). It also gives precise definition of the class of 2-complexes one should consider.

==> One vertex spin-foams with the Dipole Cosmology boundary/B_bibliografia.tex <==
\begin{thebibliography}{99}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Powyzej kreski sa prace, ktore beda cytowane w tej pracy
\bibitem{RR}
	{Reisenberger~MP}~(1994)~\emph{World sheet formulations of gauge theories and gravity}, {} {(\emph{Preprint} arXiv:gr-qc/9412035)}\\
	Reisenberger~MP, Rovelli~C~(1997)~\emph{``Sum over Surfaces'' form of Loop Quantum Gravity}, {Phys.Rev.}{\bf D56},{3490-3508} {(\emph{Preprint} arXiv:gr-qc/9612035v)}
\bibitem{Baezintro}
	{Baez~J}~(2000)~\emph{An introduction to Spinfoam Models of BF Theory and Quantum Gravity}, {Lect.Notes Phys.}{\bf 543},{25-94} {(\emph{Preprint} arXiv:gr-qc/9905087v1)}
\bibitem{perez}
	{Perez~A}~(2003)~\emph{Spinfoam models for Quantum Gravity}, {Class.Quant.Grav.}{\bf 20},{R43} {(\emph{Preprint} arXiv:gr-qc/0301113v2)}
\bibitem{Rovellibook}
	{Rovelli~C}~(2004)~\emph{Quantum Gravity}, {(Cambridge: Cambridge University Press)}
\bibitem{Operator_SF}
	{Bahr~B, Hellmann~F, Kami\'nski~W, Kisielowski~M, Lewandowski~J}~(2010)~\emph{Operator Spin Foam Models}, {Class.Quant.Grav.}{\bf 28},{105003,2011} {(\emph{Preprint} arXiv:1010.4787v1)}
\bibitem{AshLewrev}
	{Ashtekar~A, Lewandowski~J}~(2004)~\emph{Background independent quantum gravity: A status report}, {Class.Quant.Grav.}{\bf 21},{R53} {(\emph{Preprint} arXiv:gr-qc/0404018)}
\bibitem{Marev}
	{Muxin~Han, Weiming~Huang, Yongge~Ma}~(2007)~\emph{Fundamental Structure of Loop Quantum Gravity}, {Int.J.Mod.Phys.}{\bf D16},{1397-1474} {(\emph{Preprint} arXiv:gr-qc/0509064)}
\bibitem{Ashtekarbook}
	{Ashtekar~A}~(1991)~\emph{Lectures on Non-perturbative Canonical Gravity}, {(Notes prepared in collaboration with R.S. Tate), (World Scientific Singapore)}
\bibitem{Thiemannbook}
	{Thiemann~T}~(2007)~\emph{Introduction to Modern Canonical Quantum General Relativity}, {(Cambridge: Cambridge University Press)}
\bibitem{LQGdiscr}
	{Rovelli~C, Smolin~C}~(1995)~\emph{Discreteness of area and volume in quantum gravity}, {Nucl.Phys.}{\bf B442},{593 [(1995) Erratum-ibid. \textbf{B456}  753]}  {(\emph{Preprint} arXiv:gr-qc/9411005)}\\
	{Ashtekar~A, Lewandowski~J}~(1995)~\emph{Differential Geometry on the Space of Connections via Graphs and Projective Limits}, {J.Geom.Phys.}{\bf 17},{191-230} {(\emph{Preprint} arXiv:hep-th/9412073)}\\
	{Ashtekar~A, Lewandowski~J}~(1997)~\emph{Quantum theory of geometry. I: Area operators}, {Class.Quant.Grav.}{\bf 14},{A55} {(\emph{Preprint} arXiv:gr-qc/9602046)}\\
	{Ashtekar~A, Lewandowski~J}~(1998)~\emph{Quantum theory of geometry. II: Volume operators}, {Adv.Theor.Math.Phys.}{\bf 1},{388} {(\emph{Preprint} arXiv:gr-qc/9711031)}\\ 
	{Thiemann~T}~(1998)~\emph{A length operator for canonical quantum gravity}, {J.Math.Phys.}{\bf 39},{3372} {(\emph{Preprint} arXiv:gr-qc/9606092)}
\bibitem{BC}
	{Barrett~JW, Crane~L}~(1998)~\emph{Relativistic spin-networks and quantum gravity}, {J.Math.Phys.}{\bf 39},{3296-3302} {(\emph{Preprint} arXiv:gr-qc/9709028)}
\bibitem{EPRL}
	{Engle~J, Livine~E, Pereira~R, Rovelli~C}~(2008)~\emph{LQG vertex with finite Immirzi parameter}, {Nucl.Phys.}{\bf B799},{136-149} {(\emph{Preprint} arXiv:0711.0146v2)}
\bibitem{flipped}
	{Engle~J, Pereira~R, Rovelli~C}~(2008)~\emph{Flipped spinfoam vertex and loop gravity}, {Nucl.Phys.}{\bf B798},{251-290} {(\emph{Preprint} arXiv:0708.1236v1)}\\
	{Livine~ER, Speziale~S}~(2007)~\emph{A new spinfoam vertex for quantum gravity}, {Phys.Rev.}{\bf D76},{084028} {(\emph{Preprint} arXiv:0705.0674v2)}
\bibitem{FK}
	{Freidel~L, Krasnov~K}~(2008)~\emph{A New Spin Foam Model for 4d Gravity}, {Class.Quant.Grav.}{\bf 25},{125018} {(\emph{Preprint} arXiv:0708.1595v2)}\\
	{Livine~ER, Speziale~S}~(2008)~\emph{Consistently Solving the Simplicity Constraints for Spinfoam Quantum Gravity}, {Europhys.Lett.}{\bf 81},{50004} {(\emph{Preprint} arXiv:0708.1915)}\\
	{Bojowald~M, Perez~A}~(2010)~\emph{Spin foam quantization and anomalies}, {Gen.Rel.Grav.}{\bf 42},{877-907} {(\emph{Preprint} arXiv:gr-qc/0303026)}
\bibitem{HT}
	{Muxin~H, Thiemann~T}~(2010)~\emph{Commuting Simplicity and Closure Constraints for 4D Spin Foam Models}, {}{(\emph{Preprint} arXiv:1010.5444)}
\bibitem{You} {Ding~Y, Muxin H, Rovelli~C}~(2011) \emph{Generalized Spinfoams}, {Phys. Rev. D}{\bf 83} {124020}
\bibitem{E}
  {Engle~J}~(2011)~\emph{A proposed proper EPRL vertex amplitude}, {}{(\emph{Preprint} arXiv:1111.2865)}
  {Engle~J}~(2012)~\emph{A spin-foam vertex amplitude with the correct semiclassical limit}, {}{(\emph{Preprint}  arXiv:1201.2187)}
\bibitem{SFLQG}
	{Kami\'nski~W, Kisielowski~M, Lewandowski~J}~(2010)~\emph{Spin-Foams for All Loop Quantum Gravity}, {Class.Quantum~Grav.}{\bf 27},{095006} {(\emph{Preprint} arXiv:0909.0939v2)}
\bibitem{FrankPhD}
	{Hellmann~F}~(2011)~\emph{State Sums and Geometry}, {PhD Thesis} University of Nottingham {(\emph{Preprint} arXiv:1102.1688v1)}
\bibitem{OSD}
	{Kisielowski~M, Lewandowski~J, Puchta~J}~(2012)~\emph{Feynman diagrammatic approach to spinfoams },{Class. Quantum Grav.}{\bf 29} 015009 {(\emph{Preprint} arXiv:1107.5185v1}
\bibitem{SF_cosmology}
	{Bianchi~E, Rovelli~C, Vidotto~F}~(2010)~\emph{Towards Spinfoam Cosmology}, {Phys.Rev.}{\bf D82},{084035,2010} {(\emph{Preprint} arXiv:1003.3483v1)}

\end{thebibliography}


